On the Transversal Number and VC-Dimension of Families of Positive Homothets of a Convex Body

Let F be a family of positive homothets (or translates) of a given convex body K in R^n. We investigate two approaches to measuring the complexity of F. First, we find an upper bound on the transversal number $\tau(F)$ of F in terms of $n$ and the independence number $\nu(F)$. This question is motivated by a problem of Gr\"unbaum. Our bound $\tau(F)\le 2^n \binom{2n}{n} (n \log n + \log\log n + 5n) \nu(F)$ is exponential in n, an improvement from the previously known bound of Kim, Nakprasit, Pelsmajer and Skokan, which was of order n^n. By a lower bound, we show that the right order of magnitude is exponential in n. Next, we consider another measure of complexity, the Vapnik--Chervonenkis dimension of F. We prove that this quantity is at most 3 if n=2 and is infinite for some F if n>2. This settles a conjecture of G\"unbaum: Show that the maximum dual VC-dimension of a family of positive homothets of a given convex body K in R^n is n+1. This conjecture was disproved by Naiman and Wynn, who constructed a counterexample of dual VC-dimension $\lfloor 3n/2\rfloor$. Our result implies that no upper bound exists.

==> Makefile <==
name=MNST
default: $(name).pdf
.PHONY: default
cleanable += $(foreach ext,pdf log aux bbl blg out spl,$(name).$(ext))
cleanable += *.pyc
cleanable += *-fig.pdf *-fig.eps *-fig.tex

MNST.tar.gz: MNST.pdf conv-fig.pdf quad-fig.pdf paraboloid-fig.pdf
	tar zcvf $@ MNST.tex MNST.bbl Makefile \
	    conv.py quad.py base.py paraboloid.py enkidu.py \
	    conv-fig.pdf quad-fig.pdf paraboloid-fig.pdf \
	    conv-frag.tex quad-frag.tex paraboloid-frag.tex
cleanable += MNST.tar.gz

PDFLATEX = pdflatex -halt-on-error -interaction nonstopmode -file-line-error
$(name).pdf: $(name).tex conv-fig.pdf quad-fig.pdf paraboloid-fig.pdf biblio.bib
	rm -f $(name).bbl
	$(PDFLATEX) $<
	if grep '^No file $(name).bbl.$$' $(name).log; then \
	    bibtex $(name) && $(PDFLATEX) $<; fi
	while grep Rerun $(name).log >/dev/null; do \
	    $(PDFLATEX) $< ; \
	done
	if grep "undefined references" $(name).log; then false; fi

conv-fig.eps: base.py
quad-fig.eps: base.py

# Convert figure bar.eps to bar.pdf.
# (We have to do this because pdflatex insists on PDF figures.)
# (We can't run epstopdf alone because it mungs the status code from
# ghostscript when there's an error, and we can't run ps2pdf alone
# because it gets the bounding box wrong.  The combination of the
# two seems to work well enough.)
%.pdf: %.eps
	epstopdf --nogs $< |ps2pdf - $@

# Run Enkidu source file bar.py to generate figure bar-fig.{eps,tex}.
%-fig.eps %-frag.tex: %.py enkidu.py
	python $< $*-fig pdf
	mv $*-fig.tex $*-frag.tex  # because arXiv doesn't like foo.{tex,pdf}

.PHONY: clean
clean:
	rm -f $(cleanable)


==> conv-frag.tex <==
\setlength{\unitlength}{1bp}%
\begin{picture}(168,168)
\put(0,0){\includegraphics{conv-fig.pdf}}
\put(84.000000,123.000000){\makebox(0,0)[b]{$x_1$}}
\put(45.000000,70.000000){\makebox(0,0)[b]{$x_2$}}
\put(102.000000,44.000000){\makebox(0,0)[t]{$x_3$}}
\put(124.000000,84.000000){\makebox(0,0)[l]{$x_4$}}
\put(10.585786,64.585786){\makebox(0,0)[tr]{$p$}}
\put(42.214214,28.585786){\makebox(0,0)[tl]{$T^{-1}x_2$}}
\end{picture}


==> paraboloid-frag.tex <==
\setlength{\unitlength}{1bp}%
\begin{picture}(312,162)
\put(0,0){\includegraphics{paraboloid-fig.pdf}}
\end{picture}


==> quad-frag.tex <==
\setlength{\unitlength}{1bp}%
\begin{picture}(168,168)
\put(0,0){\includegraphics{quad-fig.pdf}}
\put(84.000000,123.000000){\makebox(0,0)[b]{$x_1$}}
\put(45.000000,70.000000){\makebox(0,0)[b]{$x_2$}}
\put(102.000000,44.000000){\makebox(0,0)[t]{$x_3$}}
\put(124.000000,84.000000){\makebox(0,0)[l]{$x_4$}}
\put(13.414214,46.414214){\makebox(0,0)[bl]{$A$}}
\put(154.000000,109.941176){\makebox(0,0)[r]{$B$}}
\put(84.000000,154.000000){\makebox(0,0)[t]{$C$}}
\put(88.500000,79.500000){\makebox(0,0)[None]{$D$}}
\put(92.470588,14.000000){\makebox(0,0)[b]{$E$}}
\end{picture}

